Sparse Estimation using Bayesian Hierarchical Prior Modeling for Real and Complex Linear Models

In sparse Bayesian learning (SBL), Gaussian scale mixtures (GSMs) have been used to model sparsity-inducing priors that realize a class of concave penalty functions for the regression task in real-valued signal models. Motivated by the relative scarcity of formal tools for SBL in complex-valued models, this paper proposes a GSM model - the Bessel K model - that induces concave penalty functions for the estimation of complex sparse signals. The properties of the Bessel K model are analyzed when it is applied to Type I and Type II estimation. This analysis reveals that, by tuning the parameters of the mixing pdf different penalty functions are invoked depending on the estimation type used, the value of the noise variance, and whether real or complex signals are estimated. Using the Bessel K model, we derive a sparse estimator based on a modification of the expectation-maximization algorithm formulated for Type II estimation. The estimator includes as a special instance the algorithms proposed by Tipping and Faul [1] and by Babacan et al. [2]. Numerical results show the superiority of the proposed estimator over these state-of-the-art estimators in terms of convergence speed, sparseness, reconstruction error, and robustness in low and medium signal-to-noise ratio regimes.

==> abl_app.tex <==
This appendix contains the computation of the quantities used in Section~\ref{subsec:fastscheme}.

\subsection{Computation of $\langle|w_i|\rangle$ \label{app:sbl_wi}}

We follow the approach in \citet{ShutinFastRVM} in order to compute $\langle|w_i|^2\rangle$. We can express $\langle|w_i|^2\rangle$ as $\langle|w_i|^2\rangle = \ev^\trans_i(\Sigmamathat + \muvhat\muvhat^\hermit)\ev_i$ with $\ev_i$ being an $N\times1$ vector of all zeros with $1$ at the $i$th position. First, we consider the dependency of $\Sigmamathat$ in \eqref{eq:wcov} on a single parameter $\gammahat_i$. We note that $\Sigmamathat=(\lambdahat\Hmat^\hermit\Hmat+\sum_{k\neq i}\gammahat_k^{-1}\ev_k\ev_k^\trans+\gammahat_i^{-1}\ev_i\ev_i^\trans)^{-1}$. Making use of the matrix inversion lemma \citep{Mardia1979} we recast $\Sigmamathat$ as 
\begin{align} % \triangleq [0,\ldots,0,1,0,\ldots,0]^\trans
	\Sigmamathat=\Sigmamathat_{-i}-\frac{\Sigmamathat_{-i}\ev_i\ev_i^\trans\Sigmamathat_{-i}}{\gammahat_i+\ev_i^\trans\Sigmamathat_{-i}\ev_i},
\end{align}
where $\Sigmamathat_{-i}\triangleq (\lambdahat \Hmat^\hermit\Hmat+\sum_{k\neq i}\gammahat_k^{-1}\ev_k\ev_k^\trans)^{-1}$. After some straightforward algebraic manipulations,  $\langle|w_i|^2\rangle$ can be expressed as 
\begin{align}
\langle|w_i|^2\rangle = \frac{\gammahat_i^2(s_i+|q_i|^2)+\gammahat_is_i^2}{(\gammahat_i+s_i)^2}
\label{eq:wi}
\end{align} 
with the definitions $s_i \triangleq \ev_i^\trans\Sigmamathat_{-i}\ev_i$ and $q_i \triangleq \lambdahat\ev_i^\trans\Sigmamathat_{-i}\Hmat^\hermit\y$.

%Finally, by substituting \eqref{eq:wi} into \eqref{eq:gamma_mode} we obtain that if $\gammatilde_i$ exists it equals a positive solution to the cubic equation:
%\begin{align}
%0 = \eta\gamma_i^3+\gamma_i^2[2\eta s_i-(\epsilon-\rho-1)]+\gamma_i[\eta s_i^2 -2(\epsilon-\rho-1)s_i-\rho(s_i+|q_i|^2)]-(\epsilon-1)s_i^2.
%\label{eq:cubic}
%\end{align}
%When $\gamma_i$ ranges through $\mathbb{R}$, \eqref{eq:cubic} has three solutions which can be determined analytically.  
%%While a feasible update for $\gammahat_i$ is constrained to be positive, 

\subsection{Computation of the stationary points of $\ell(\gamma_i)$ \label{app:sbl_ell}}
%If positive solutions exist, a further analysis is needed to determine which of these to select for $\gammatilde$. For doing so, we show that the positive solutions of \eqref{eq:cubic} are in fact the stationary points of
We define $\ell(\gamma_i)$ according to 
\begin{align}
\ell(\gamma_i) \propto^{e} \log(p(\y|\gamma_i,\gamhat_{-i},\lambdahat)p(\gamma_i)). \label{eq:ell_gammai}
\end{align}
Following the steps in \citet{Tipping2003} we can write $\ell(\gamma_i)$ as
\begin{align}
\ell(\gamma_i) \triangleq -\rho\log|1+\gamma_i\tilde{s}_i| + \rho \frac{|\tilde{q}_i|^2}{\gamma_i^{-1}+\tilde{s}_i} + (\epsilon-1) \log \gamma_i - \eta\gamma_i
	\label{eq:lgammai}
\end{align}
with the definitions $\tilde{s}_i \triangleq \h_i^\hermit\matr{C}^{-1}_{-i}\h_i$, $\tilde{q}_i \triangleq \y^\hermit\matr{C}^{-1}_{-i}\h_i$, and $\matr{C}_{-i}\triangleq \lambdahat^{-1}\matr{I}+\sum_{k\neq i}\gammahat_k\h_k\h_k^\hermit$. Taking the derivative of $\ell$ with respect to $\gamma_i$ and equating the result to zero yields 
\begin{align}
	0 &= \eta \tilde{s}_i^2\gamma_i^3 + \gamma_i^2[ 2\eta \tilde{s}_i - (\epsilon-\rho-1)\tilde{s}_i^2 ] + \gamma_i [ \eta +\rho(\tilde{s}_i - |\tilde{q}_i|^2)- 2(\epsilon-1)\tilde{s}_i ] - (\epsilon-1). 
	\label{eq:cubic2}
\end{align} 
Making use of the matrix inversion lemma for $\matr{C}^{-1}_{-i}$, we show the identities $s_i = \tilde{s}^{-1}_i$ and $|q_i|^2 = |\tilde{q}_i|^2/\tilde{s}_i^2$ \citep{ShutinFastRVM}. By substituting these identities into \eqref{eq:cubic}, we arrive at the cubic equation in \eqref{eq:cubic2}. This verifies that the positive solutions of \eqref{eq:cubic} are the stationary points of $\ell$. 
%Thus, we simply select the $\gammatilde_i$ that maximizes $\ell$ among the positive solutions of \eqref{eq:cubic}. With this important result, we consider several different choices for $\epsilon$ and $\eta$. Some particular parameters settings reveal the direct relationship of our proposed fast algorithm to the fast algorithms in \citet{Tipping2003} and \citet{Babacan2010}. %For simplicity, we let $\gammahat_i= \gammahat_i^{[\infty]}$ throughout the rest of the section.


==> app_algorithm.tex <==
\setcounter{thmcounter}{0}
We start out by computing the derivative of $\ell(\gamma_i)$ (see \eqref{eq:lgammal}):
\begin{align}
 \ell'(\gamma_i) = \frac{-\gamma_i^2\hat{\eta}_i s_i^2 - \gamma_i\big[ (1-\epsilon+\rho)s_i^2 + 2\hat{\eta}_i s_i \big] + \big[ 2(\epsilon-1)s_i - s_i\rho + \rho |q_i|^2 - \hat{\eta}_i \big] + \gamma_i^{-1}(\epsilon-1)}{ (1+\gamma_is_i)^2}.
	\label{eq:dlgammal}
\end{align}
%As the function $\ell'(\gamma_i)$ has a singularity in $\gamma_i=0$ and $(1+\gamma_is_i)^2 > 0$, 
For the proofs of Propositions~\ref{thm:thm1} and \ref{thm:thm3} we define the function $f(\gamma_i) \triangleq \gamma_i(1+\gamma_is_i)^2\ell'(\gamma_i)$ corresponding to the right-hand polynomial in \eqref{eq:cubic}:
\begin{align}
	f(\gamma_i) = -\gamma_i^3\hat{\eta}_i s_i^2 - \gamma_i^2\big[ (1-\epsilon+\rho)s_i^2 + 2\hat{\eta}_i s_i \big] + \gamma_i \big[ 2(\epsilon-1)s_i - s_i\rho + \rho |q_i|^2 - \hat{\eta}_i \big] + (\epsilon-1).
	\label{eq:cubic_app}
\end{align}
Notice that: (i) $\ell'(\gamma_i)$ and $f(\gamma_i)$ share the same roots on $\mathbb{R}^+$ corresponding to the stationary points of $\ell(\gamma_i)$; (ii) For any positive $\gamma_i$, $\ell'(\gamma_i)$ and $f(\gamma_i)$ have the same sign. Hence, we can study the stationary points of $\ell(\gamma_i)$ from the analysis of $f(\gamma_i)$ on $\mathbb{R}^+$. Finally, the derivative of $f(\gamma_i)$,
\begin{align}
	f'(\gamma_i)=-3\gamma_i^2\hat{\eta}_i s_i^2 - 2\gamma_i\big[ (1-\epsilon+\rho)s_i^2 + 2\hat{\eta}_i s_i \big] + \big[ 2(\epsilon-1)s_i - s_i\rho + \rho |q_i|^2 - \hat{\eta}_i \big],
	\label{eq:cubicDeriv}
\end{align}
is a concave parabola that crosses the $\gamma_i$-axis at the two points
\begin{align}
	\gamma_i^{(-)} &= \frac{-s_i^2(1-\epsilon+\rho)-2s_i\hat{\eta}_i-s_i\sqrt{d_i}}{3s_i^2\hat{\eta}_i},\label{eq:crossingpoints1}\\
	\gamma_i^{(+)} &= \frac{-s_i^2(1-\epsilon+\rho)-2s_i\hat{\eta}_i+s_i\sqrt{d_i}}{3s_i^2\hat{\eta}_i}.\label{eq:crossingpoints2}
\end{align} 
Here, $d_i\triangleq s_i^2(1-\epsilon+\rho)^2-2s_i\hat{\eta}_i+s_i\hat{\eta}_i(2\epsilon+\rho)+\hat{\eta}_i(\hat{\eta}_i+3|q_i|^2\rho)$. Note that $\gamma_i^{(-)}$ is either complex (and so is $\gamma_i^{(+)}$) or negative for $\epsilon\leq 1+\rho$. 

We begin by analyzing the case in which $\epsilon<1$, as assumed in Proposition~\ref{thm:thm1}. We will need the following lemma:

\begin{lemma}\label{thm:lemmaA1}
	Provided $\epsilon<1$, if the function $f(\gamma_i)$ has positive roots then it has exactly two of them.
\end{lemma}
\begin{IEEEproof}
  Assume that $\epsilon<1$. As $f(0) = \epsilon-1 <0$ and $\lim_{\gamma_i\rightarrow-\infty}f(\gamma_i)=\infty$, $f(\gamma_i)$ has an odd number of negative roots (either one or three). Hence, if  $f(\gamma_i)$ has positive roots it must have exactly two of them.
\end{IEEEproof}

Using Lemma~\ref{thm:lemmaA1} we can now prove Proposition~\ref{thm:thm1}.
\begin{thm}
Provided $\epsilon<1$ the function $\ell(\gamma_i)$ has at most a single local maximum.        
\end{thm}
\begin{IEEEproof}
Assume that $\epsilon<1$. From Lemma~\ref{thm:lemmaA1}, $f(\gamma_i)$ has either exactly two positive roots $\gamma_i^{(1)}$ and $\gamma_i^{(2)}$, or it has no such root at all.
In the latter case $\ell(\gamma_i)$ has no local maximum.\footnote{Remember that the definition domain of $\ell(\gamma_i)$ is $\mathbb{R}^+$.} In the former case, we distinguish between two different possibilities: (i) $\gamma_i^{(1)} = \gamma_i^{(2)} = \gamma^{(+)}$ and (ii) $0 <\gamma_i^{(1)}<\gamma^{(+)}<\gamma_i^{(2)}$. If (i) holds true,  $\gamma_i^{(1)} = \gamma_i^{(2)} = \gamma^{(+)}$ corresponds to a saddle point of $\ell(\gamma_i)$. 
Indeed, since $f(0) = (\epsilon-1)<0$ and  $\lim_{\gamma_i\rightarrow\infty}f(\gamma_i)=-\infty$, $\gamma_i^{(1)} = \gamma_i^{(2)} = \gamma^{(+)}$ corresponds to the maximum of $f(\gamma_i)$ and, hence, $f(\gamma_i)$ is negative on both intervals $(0,\gamma_i^{(+)})$ and $(\gamma_i^{(+)},\infty)$. 
This implies that $\ell(\gamma_i)$ monotonically decreases on these two intervals, hence, $\gamma_i^{(+)}$ corresponds to a saddle point of $\ell(\gamma_i)$. 
If (ii) holds true, the rightmost root $\gamma_i^{(2)}$ must necessarily correspond to a local maximum. 
Since $f'(\gamma_i)$ is a concave parabola with $d_i>0$ and $f(0)<0$, the function $\ell(\gamma_i)$ decreases on the interval $(0,\gamma_i^{(1)})$ because $f(\gamma_i)$ is negative on this interval, then increases on $(\gamma_i^{(1)}, \gamma_i^{(2)})$ as $f(\gamma_i)$ is positive on this interval, and finally decreases towards $-\infty$ on the interval $(\gamma_i^{(2)}, \infty)$. 
Thus, $\gamma_i^{(1)}$ corresponds to the local minimum of $\ell(\gamma_i)$ and $\gamma_i^{(2)}$ corresponds to the only local maximum of $\ell(\gamma_i)$.
\end{IEEEproof}

We now turn to the proof of Proposition~\ref{thm:thm3}. We begin by proving the following lemma:
\begin{lemma}\label{thm:lemmaA2}
 Provided $1< \epsilon\leq 1+\rho$ the function $f(\gamma_i)$ has a positive root of multiplicity one or three.
\end{lemma}
\begin{IEEEproof}
Assume $1< \epsilon\leq 1+\rho$. 
The function $f(\gamma_i)$ has at least a positive root as $f(0) = (\epsilon-1) > 0$ and $\lim_{\gamma_i\rightarrow\infty}f(\gamma_i)=-\infty$. Moreover, $f'(\gamma_i)$ can at most change sign once over $\mathbb{R}^+$ as $\gamma_i^{(-)}$ is either negative or complex for $\epsilon\leq 1+\rho$. Thus, $f(\gamma_i)$ has a positive root of multiplicity one or three.
\end{IEEEproof}

Now, we are ready to state Proposition~\ref{thm:thm3}.
\begin{thm}     
Provided $1<\epsilon\le 1+\rho$ the function $\ell(\gamma_i)$ has a single stationary point and this stationary point corresponds to a maximum.    
\end{thm}  
\begin{IEEEproof}
From Lemma~\ref{thm:lemmaA2}, $f(\gamma_i)$ has a positive root $\gamma_i^{(*)}$ of multiplicity either one or three. Hence, $\ell(\gamma_i)$ has a single stationary point. Moreover, as $f(0) = (\epsilon-1) > 0$, $f(\gamma_i)$ is positive on the interval $(0,\gamma_i^{(*)})$ and negative on the interval $(\gamma_i^{(*)},\infty)$, which implies that this stationary point corresponds to the maximum of $\ell(\gamma_i)$.
\end{IEEEproof}


==> signal_model.tex <==
We begin with the specification of the probabilistic structure of the SBL problem for signal model \eqref{eq:model}. % $\ell_1$-norm parameter constraints. 
Two types of hierarchical prior models for the weight vector $\vect{\alpha}$ are considered: a 2-L and a 3-L hierarchical model. 
Later we will see that these models lead to priors for $\vect{\alpha}$ with distinct sparsity-inducing properties.

%For the 2-L prior model the joint pdf of the signal model \eqref{eq:model} reads
The joint pdf of the signal model \eqref{eq:model} augmented with the 2-L prior model for $\vect{\alpha}$ reads
\begin{align}
p(\vect{y},\vect{\alpha},\vect{\gamma},\lambda) = p(\vect{y}|\vect{\alpha},\lambda)p(\lambda)p(\vect{\alpha}|\vect{\gamma})p(\vect{\gamma}).
%p(\vect{y},\vect{\alpha},\vect{\gamma},\vect{\eta},\lambda) = p(\vect{y}|\vect{\alpha},\lambda)p(\lambda)\prod_{l=1}^{L} p(\alpha_l|\gamma_l)p(\gamma_l)p(\eta_l),
	\label{eq:jointpdf2layer}
\end{align}
%Here $p(\vect{y}|\vect{\alpha},\lambda)$ is the likelihood function of the weights $\vect{\alpha}$ and noise precision parameter $\lambda$.
From \eqref{eq:model}, $p(\vect{y}|\vect{\alpha},\lambda)$ is Gaussian: $\GaussPDF(\vect{y}|\matr{H}\vect{\alpha},\lambda^{-1}\matr{I})$ if the signal model is real and $\CGaussPDF(\vect{y}|\matr{H}\vect{\alpha},\lambda^{-1}\matr{I})$ if it is complex.\footnote{$\GaussPDF(\cdot|\vect{a},\matr{B})$ and $\CGaussPDF(\cdot|\vect{a},\matr{B})$ denote respectively a multivariate real and a multivariate complex Gaussian pdf with mean vector $\vect{a}$ and covariance matrix $\matr{B}$.} %$p(\vect{y}|\vect{\alpha},\lambda)=\CGaussPDF(\vect{y}|\matr{H}\vect{\alpha},\lambda^{-1}\matr{I})$ for the complex model. 
%The prior $p(\lambda)$ is selected as a gamma pdf, i.e., $p(\lambda) = p(\lambda; c,d) \triangleq \GammaPDF(\lambda|c,d)$.
%This choice is convenient since the gamma distribution is a conjugate prior for the precision of a Gaussian likelihood function. 
%Note that the selection $c=d=0$ leads to the noninformative Jeffreys prior for the noise precision parameter.
The sparsity-inducing properties of this Bayesian model are determined by the joint prior pdf $p(\vect{\alpha}|\vect{\gamma})p(\vect{\gamma})$. 
Motivated by GSM modeling as well as previous works on SBL \cite{Tipping2001,Figueiredo,Babacan2010} we select the conditional prior pdf $p(\vect{\alpha}|\vect{\gamma})$ to factorize in a product of Gaussian pdfs: $p(\vect{\alpha}|\vect{\gamma}) = \prod_{l=1}^{L} p(\alpha_l|\gamma_l)$. % both real and complex $\vect{\alpha}$ are considered. 
For the sake of using a single notation for $p(\alpha_l|\gamma_l)$ for both real and complex weights, we introduce the parameterization
\begin{align}
p(\alpha_l|\gamma_l)=\left(\frac{\rho}{\pi\gamma_l}\right)^\rho\exp\left(-\rho\frac{|\alpha_l|^2}{\gamma_l}\right). %,\quad \rho \geq 0.
\label{eq:real_complex_gaussian}
\end{align} 
The conditional prior pdf $p(\alpha_l|\gamma_l)$ for real $\alpha_l$ is realized by selecting $\rho=1/2$, while $\rho=1$ entails the conditional prior pdf for complex $\alpha_l$. 

%While the conditional prior $p(\vect{\alpha}|\vect{\gamma})$ itself is not sparsity inducing, probabilistic modeling of $\vect{\gamma}$ leads to an equivalent model that does impose sparsity constraints. 
%For 2-L models the $\ell_1$-norm parameter constraint for real $\vect{\alpha}$ is realized by selecting $p(\vect{\gamma})\equiv p(\vect{\gamma}; \vect{\eta})$ as an exponential pdf \cite{Figueiredo} pdf with fixed parameters $\vect{\eta}$. 
%These parameters are functionally related to the regularization parameters that control the trade-off between the quadratic error $\|\vect{y}-\matr{H}\vect{\alpha}\|^2_2$ and a penalty term in \eqref{eq:map_general}.
%The proper selection of these parameters is crucial for optimal performance of the models.
%While techniques exist to empirically select regularization parameters, see, e.g., re-weighted  $\ell_1$ scheme \cite{Candes2008}, Bayesian methodology offers a consistent way to estimate $\vect{\eta}$.      
%This is realized by extending the 2-L hierarchy with an additional hierarchy tier, where the hyperprior parameters $\vect{\eta}$ are also modeled as random variables \cite{Lee2010,Babacan2010}. 
The hyperprior pdf $p(\vect{\gamma})= p(\vect{\gamma}; \vect{\eta})$ of the 2-L prior model is selected to be some suitable pdf defined over $\mathbb{R}^+$ with fixed parameter $\vect{\eta}$. %This parameter is functionally related to the regularization parameter that control the trade-off between the quadratic error $\|\vect{y}-\matr{H}\vect{\alpha}\|^2_2$ and the penalty term in \eqref{eq:map_general}. 
%This observation has motivated 
An extension of a 2-L hierarchy with an additional layer, where the entries in $\vect{\eta}$ are also modeled as random variables, has been considered in \cite{Lee2010,Babacan2010}. Doing so yields the corresponding 3-L prior model with the joint pdf specified as follows: 
\begin{align}
p(\vect{y},\vect{\alpha},\vect{\gamma},\vect{\eta},\lambda) = p(\vect{y}|\vect{\alpha},\lambda)p(\lambda)p(\vect{\alpha}|\vect{\gamma})p(\vect{\gamma}|\vect{\eta})p(\vect{\eta}),
%p(\vect{y},\vect{\alpha},\vect{\gamma},\vect{\eta},\lambda) = p(\vect{y}|\vect{\alpha},\lambda)p(\lambda)\prod_{l=1}^{L} p(\alpha_l|\gamma_l)p(\gamma_l)p(\eta_l),
	\label{eq:jointpdf1}
\end{align}
where $p(\vect{\eta})$ of $\vect{\eta}$ is the pdf of the  ''hyper-hyperprior''.
%The joint pdf of signal model \eqref{eq:model} with a 3-L prior for $\vect{\alpha}$ is obtained by assuming that the parameters $\vect{\eta}$ of the $p(\vect{\gamma})$ in \eqref{eq:jointpdf2layer} are random. 
%The resulting joint pdf is then specified as   
%\begin{align}
%p(\vect{y},\vect{\alpha},\vect{\gamma},\vect{\eta},\lambda) = p(\vect{y}|\vect{\alpha},\lambda)p(\lambda)p(\vect{\alpha}|\vect{\gamma})p(\vect{\gamma}|\vect{\eta})p(\vect{\eta}).
%p(\vect{y},\vect{\alpha},\vect{\gamma},\vect{\eta},\lambda) = p(\vect{y}|\vect{\alpha},\lambda)p(\lambda)\prod_{l=1}^{L} p(\alpha_l|\gamma_l)p(\gamma_l)p(\eta_l),
%	\label{eq:jointpdf1}
%\end{align}
%Both the 2-L formulation \eqref{eq:jointpdf2layer} and the 3-L formulation \eqref{eq:jointpdf1} share the same likelihood function $p(\vect{y}|\vect{\alpha},\lambda)$ and the prior pdf of the noise precision parameter $p(\lambda)$.
%Due to \eqref{eq:model} the likelihood function is Gaussian: $p(\vect{y}|\vect{\alpha},\lambda)=\GaussPDF(\vect{y}|\matr{H}\vect{\alpha},\lambda^{-1}\matr{I})$ for the real signal model and $p(\vect{y}|\vect{\alpha},\lambda)=\CGaussPDF(\vect{y}|\matr{H}\vect{\alpha},\lambda^{-1}\matr{I})$ for the complex model. 
%The prior $p(\lambda)$ models the distribution of the noise precision parameter $\lambda$, i.e., the inverse of the noise variance, $\lambda := \sigma^{-2}$. 

%\footnote{The gamma pdf is central for the work conducted and used throughout the paper. Specifically, for the non-negative random variable $X$ the gamma pdf is given by: $p(x;a,b) = \frac{b^a}{\Gamma(a)}x^{a-1}\exp(-bx)$, $a,b > 0$.} 
%This choice is convenient since the gamma distribution is a conjugate prior for the precision of a Gaussian likelihood function. 
%Note that the selection $c=d=0$ leads to the noninformative Jeffreys prior for the precision. % of a Gaussian random variable.
%Additionally, selecting $c=d=0$ makes this prior noninformative. 

%We now specify the structure of the hierarchical priors of $\vect{\alpha}$ in \eqref{eq:jointpdf2layer} and \eqref{eq:jointpdf1}. 
%Motivated by GSM models and the work in \cite{Tipping2001,Figueiredo} we select this conditional prior to factorize in a product of Gaussian pdfs: $p(\vect{\alpha}|\vect{\gamma}) = \prod_{l=1}^{L} p(\alpha_l|\gamma_l)$.   
%While in \cite{Tipping2001,Figueiredo} real $\vect{\alpha}$ was considered, here 
%We consider both real and complex $\vect{\alpha}$. To this end we define the parametrization
%\begin{align}
%p(\alpha_l|\gamma_l)=\left(\frac{\rho}{\pi\gamma_l}\right)^\rho\exp\left(-\rho\frac{|\alpha_l|^2}{\gamma_l}\right),\quad \rho \geq 0.
%\label{eq:real_complex_gaussian}
%\end{align} 
%with the parameter $\rho\in\{\frac{1}{2},1\}$. 
%The conditional prior $p(\alpha_l|\gamma_l)$ for real $\alpha_l$ is realized by selecting $\rho=1/2$, while $\rho=1$ entails the conditional prior for complex $\alpha_l$.
%In what follows we analyze these structures in more detail by computing equivalent priors for the weights $\vect{\alpha}$ obtained by marginalizing over the hyperparameters $\vect{\gamma}$ and $\vect{\eta}$ and discuss the required modifications of the priors to encompass real as well as complex modeling of $\ell_1$-norm parameter constraints.
In the sequel we analyze the 2-L and 3-L prior models in more detail by computing the prior pdfs of the weight vector $\vect{\alpha}$ obtained by marginalizing the joint prior pdfs $p(\vect{\alpha}|\vect{\gamma})p(\vect{\gamma})$ and $p(\vect{\alpha}|\vect{\gamma})p(\vect{\gamma}|\vect{\eta})p(\vect{\eta})$ with respect to the hyperparameters $\vect{\gamma}$ and $\{\vect{\gamma},\vect{\eta}\}$ respectively. %We then computing equivalent priors for the weights $\vect{\alpha}$ obtained by marginalizing over the hyperparameters $\vect{\gamma}$ and $\vect{\eta}$. 
We then discuss the sparsity-inducing properties of these marginalized priors in the case when the weights are real and complex. This includes the modeling of the $\ell_1$ penalty term as a special case.          
%In the next section we compute the prior for $\vect{\alpha}$ that results from the 2-L prior model and analyze its sparsity-inducing property. We redo the same exercise in Section~\ref{subsec:D3H} with the 3-L prior model.


\subsection{Two-Layer Hierarchical Prior Model \label{subsec:2L}}
\input{two_layer_model.tex}  

\subsection{Three-Layer Hierarchical Prior Model \label{subsec:3L}}
\input{three_layer_model.tex}  

%\subsection{Weighted log-sum Penalization \label{sec:NewApproach}}
%\subsection{An Informative Prior \label{sec:NewApproach}}
%\input{new_approach.tex}





